Robust Node ID Assignment for Mobile P2P Networks

The advancement of portable mobile wireless devices such as smart-phones, PDA, etc., brought mobile peer-to-peer (P2P) as an extension of traditional P2P networks to provide efficient, low-cost communication among them in a cellular network. It is challenging to assign a unique identifier to each user, as an adversary can target to disrupt the P2P system, by carefully selecting user IDs or obtaining many pseudo-IDs. This work proposes a robust node-ID assignment mechanism for secure peer joining in mobile P2P system called PJ-Sec. PJ-Sec facilitates to generate nodeID for a joining peer by a collaborative effort of an existing peer (within the vicinity) and pre-selected vicinity head. PJ-Sec is formally analyzed using AVISPA model checker and found to be attack resistant.

==> lookupNew.tex <==
\RestyleAlgo{boxruled}
%\LinesNumbered
\begin{algorithm}  [!ht]
\normalsize
\caption{(Lookup in V-Chord.)} \label{RoutingAlg:3} 

$ID_{[i..j]}$ denotes the overlay ID from $i^{th}$ to $j^{th}$ bit.

Each key K to be forwarded to exact or closest $ID_{[i..j]}$ during lookup.

\textbf{dMS:}

$dMS_a$ requests a key $K_a$ to associate pilot dMS$_a^P$.

\textbf{Pilot:}

Pilot dMS$_a^P$ searches $K_{a[1..m]}$  in its GTable)

\If {($K_{a[1..m]}$ == GTable.dMS$_{[1..m]}$)} { // say $dMS_i$

Reply $dMS_i$ to $dMS_a$ 

}

\Else{

	\If {($K_{a[1..p]}$ == GTable.dMS$_{[1..p]}$)} { // say $dMS_i^P$

		Forwards the request to $dMS_i^P$ 
		
		}

}
\Else{

	Forwards the request to  the nearest $dBTS$

}

\textbf{BTS:}

$K_{a[1..b]}$ forwards the request to nearest BTS dBTSID$_{a[1..b]}$ (say $dBTS_i$) , which forwards to an appropriate pilot.
   
\end{algorithm}


